Heterogeneous-Reliability Memory: Exploiting Application-Level Memory Error Tolerance

This paper summarizes our work on characterizing application memory error vulnerability to optimize datacenter cost via Heterogeneous-Reliability Memory (HRM), which was published in DSN 2014, and examines the work's significance and future potential. Memory devices represent a key component of datacenter total cost of ownership (TCO), and techniques used to reduce errors that occur on these devices increase this cost. Existing approaches to providing reliability for memory devices pessimistically treat all data as equally vulnerable to memory errors. Our key insight is that there exists a diverse spectrum of tolerance to memory errors in new data-intensive applications, and that traditional one-size-fits-all memory reliability techniques are inefficient in terms of cost. This presents an opportunity to greatly reduce server hardware cost by provisioning the right amount of memory reliability for different applications. Toward this end, in our DSN 2014 paper, we make three main contributions to enable highly-reliable servers at low datacenter cost. First, we develop a new methodology to quantify the tolerance of applications to memory errors. Second, using our methodology, we perform a case study of three new data-intensive workloads (an interactive web search application, an in-memory key--value store, and a graph mining framework) to identify new insights into the nature of application memory error vulnerability. Third, based on our insights, we propose several new hardware/software heterogeneous-reliability memory system designs to lower datacenter cost while achieving high reliability and discuss their trade-offs. We show that our new techniques can reduce server hardware cost by 4.7% while achieving 99.90% single server availability.

==> Makefile <==
################################################################################
# Custom Rules
################################################################################

SRC  = $(shell egrep -l '^[^%]*\\begin\{document\}' *.tex)
TRG  = $(SRC:%.tex=%.pdf)

all: $(TRG)
.PHONY: $(TRG) clean rolling

################################################################################
# Latexmk Rules
################################################################################
# -pdf: Generate pdf version of document using pdflatex.
#
# -bibtex: When the source file uses bbl files for bibliography, run bibtex or
#  biber as needed to regenerate the bbl files.
#
#  -C: Clean up (remove) all regeneratable files generated by latex and bibtex
#  or biber.
################################################################################

rolling: $(SRC)
	latexmk -pvc -pdf -bibtex -interaction=nonstopmode $(SRC)

$(TRG): $(SRC) *.tex
	latexmk -pdf -bibtex $(SRC)

clean:
	latexmk -c -bibtex



==> websearch-mapping-table.tex <==
%\begin{table*}
%\footnotesize
%\tabcolsep=0.1cm
%\begin{center}
%%\rule[-16.4mm]{0.3mm}{34.2mm}
%%\hspace{-1.5mm}
%%\begin{tabular}{m{4.5cm}}
%%\toprule
%%\centering Design parameters \tabularnewline \midrule
%%DRAM/server HW cost \hfill 30\% \tabularnewline
%%NoECC memory cost savings \hfill 11.1\% \tabularnewline
%%Parity memory cost savings \hfill 9.7\% \tabularnewline
%%L memory cost savings \hfill 18\%$\pm$12\% \tabularnewline
%%Crash recovery time \hfill 10 mins \tabularnewline
%%Par+R flush threshold \hfill 5 mins \tabularnewline
%%Errors/server/month~\cite{Schroeder09} \hfill 2000 \tabularnewline
%%Target single server availability \hfill 99.9\% \tabularnewline \bottomrule
%%\end{tabular}
%%\hspace{-1.5mm}
%%\rule[-16.4mm]{0.3mm}{34.2mm}
%%\tabcolsep=0.1cm
%\begin{tabular}{m{2cm}>{\centering}m{0.8cm}<{\centering}>{\centering}m{0.8cm}<{\centering}>{\centering}m{0.8cm}<{\centering}>{\centering}m{1.85cm}<{\centering}>{\centering}m{1.58cm}<{\centering}>{\centering}m{0.8cm}<{\centering}>{\centering}m{1.2cm}<{\centering}>{\centering}m{1.3cm}<{\centering}}
%\toprule
%\multirow{5}{*}{Configuration} & \multicolumn{3}{c}{Mapping} & \multicolumn{5}{c}{Metrics} \tabularnewline \cmidrule(lr){2-4} \cmidrule(lr){5-9}
% & Private (36GB) & Heap (9GB) & Stack (60MB) & Memory cost savings (\%) & Server HW~cost savings~(\%) & Crashes/ server/ month & Single server~availability & \#~incorrect/ million queries \tabularnewline \midrule
%Typical Server & ECC & ECC & ECC & 0.0 & 0.0 & 0 & 100.00\% & 0 \tabularnewline
%Consumer PC & NoECC & NoECC & NoECC & 11.1 & 3.3 & 19 & 99.55\% & 33 \tabularnewline
%Detect\&Recover & Par+R & NoECC & NoECC & 9.7 & 2.9 & 3 & 99.93\% & 9 \tabularnewline
%Less-Tested (L) & NoECC & NoECC & NoECC & 27.1 (16.4-37.8) & 8.1 (4.9-11.3) & 96 & 97.78\% & 163 \tabularnewline
%Detect\&Recover/L & ECC & Par+R & NoECC & 15.5 (3.1-27.9) & 4.7 (0.9-8.4) & 4 & 99.90\% & 12 \tabularnewline \bottomrule
%\end{tabular}
%\caption{
%Mapping of WebSearch address space to different hardware/software
%design points and the corresponding trade-off in cost, single server
%availability, and reliability. (ECC = SEC-DED memory; NoECC = no
%detection/correction; Par+R = parity memory and recovery from disk; L =
%less-tested memory.)
%}
%\label{tbl:search-mapping}
%\end{center}
%\end{table*}

\begin{table*}
\small
%\footnotesize
\tabcolsep=0.1cm
\begin{center}
\begin{tabular}{m{2.8cm}>{\centering}m{1.1cm}<{\centering}>{\centering}m{1.1cm}<{\centering}>{\centering}m{1.1cm}<{\centering}>{\centering}m{2.6cm}<{\centering}>{\centering}m{2cm}<{\centering}>{\centering}m{1.2cm}<{\centering}>{\centering}m{1.5cm}<{\centering}>{\centering}m{1.8cm}<{\centering}}
\toprule
\multirow{5}{*}{Configuration} & \multicolumn{3}{c}{Mapping} & \multicolumn{5}{c}{Metrics} \tabularnewline \cmidrule(lr){2-4} \cmidrule(lr){5-9}
 & Private (36GB) & Heap (9GB) & Stack (60MB) & Memory cost savings (\%) & Server HW~cost savings~(\%) & Crashes/ server/ month & Single server~availability & \#~incorrect/ million queries \tabularnewline \midrule
Typical Server & ECC & ECC & ECC & 0.0 & 0.0 & 0 & 100.00\% & 0 \tabularnewline
Consumer PC & NoECC & NoECC & NoECC & 11.1 & 3.3 & 19 & 99.55\% & 33 \tabularnewline
Detect\&Recover & Par+R & NoECC & NoECC & 9.7 & 2.9 & 3 & 99.93\% & 9 \tabularnewline
Less-Tested (L) & NoECC & NoECC & NoECC & 27.1 (16.4-37.8) & 8.1 (4.9-11.3) & 96 & 97.78\% & 163 \tabularnewline
Detect\&Recover/L & ECC & Par+R & NoECC & 15.5 (3.1-27.9) & 4.7 (0.9-8.4) & 4 & 99.90\% & 12 \tabularnewline \bottomrule
\end{tabular}
\caption{
Mapping of WebSearch address space to different hardware/software
design points and the corresponding trade-off in cost, single server
availability, and reliability. (ECC = SEC-DED memory; NoECC = no
detection/correction; Par+R = parity memory and recovery from disk; L =
less-tested memory.)
}
\label{tbl:search-mapping}
\end{center}
\end{table*}



